Vulnerability Detection with Graph Simplification and Enhanced Graph Representation Learning

Prior studies have demonstrated the effectiveness of Deep Learning (DL) in automated software vulnerability detection. Graph Neural Networks (GNNs) have proven effective in learning the graph representations of source code and are commonly adopted by existing DL-based vulnerability detection methods. However, the existing methods are still limited by the fact that GNNs are essentially difficult to handle the connections between long-distance nodes in a code structure graph. Besides, they do not well exploit the multiple types of edges in a code structure graph (such as edges representing data flow and control flow). Consequently, despite achieving state-of-the-art performance, the existing GNN-based methods tend to fail to capture global information (i.e., long-range dependencies among nodes) of code graphs. To mitigate these issues, in this paper, we propose a novel vulnerability detection framework with grAph siMplification and enhanced graph rePresentation LEarning, named AMPLE. AMPLE mainly contains two parts: 1) graph simplification, which aims at reducing the distances between nodes by shrinking the node sizes of code structure graphs; 2) enhanced graph representation learning, which involves one edge-aware graph convolutional network module for fusing heterogeneous edge information into node representations and one kernel-scaled representation module for well capturing the relations between distant graph nodes. Experiments on three public benchmark datasets show that AMPLE outperforms the state-of-the-art methods by 0.39%-35.32% and 7.64%-199.81% with respect to the accuracy and F1 score metrics, respectively. The results demonstrate the effectiveness of AMPLE in learning global information of code graphs for vulnerability detection.

==> figures/code_example.tex <==

% \begin{figure}[t]
% \centering
% \begin{lstlisting}[language=c++, numbers=left,
% basicstyle=\ttfamily,
% columns=flexible,
% keywordstyle=\color{blue!70},
% commentstyle=\color{red!50!green!50!blue!50}, 
% frame=shadowbox, 
% rulesepcolor=\color{red!20!green!20!blue!20}, 
% xleftmargin=2em,
% xrightmargin=1em, 
% aboveskip=2em,
% showstringspaces=false,
% escapeinside=``,
% emph={malloc,main,scanf,strcpy}, 
%     emphstyle={\color{blue!20!black!30!green}} ,
% ]
% void main(int `\textbf{argc}`){
%         char * `\textbf{first}` = malloc(10);
% 	char `\textbf{str}`[15];
% 	scanf("%s", `\textbf{str}`);
% 	if(`\textbf{argc}` > 1){
% 	    strcpy(`\textbf{first}`, `\textbf{str}`);	
% 	}
% }
% \end{lstlisting}
% \caption{Code Example with Buffer Overflow.}
% \label{source_code1}

% \end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width=0.35\textwidth]{figures/code_example_cropped.pdf}
%\vspace{-2ex}
\caption{Code Example with Buffer Overflow.}
\label{source_code}
\end{figure}

==> sections/discussion_old.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.49\textwidth]{figures/vul_example3_cropped.pdf}
\vspace{-2ex}
\caption{A heatmap of the CEW-77~\cite{CWE-77} example correctly predicted by \tool. The color-shaded of a statement is drawn according to the `attention' weight. Green-shaded indicates the minimum attention weight. The redder the color, the greater the `attention' weight. Red colored code are vulnerable.}% A heatmap case of the concern weights of CWE-77 successfully detected by \tool. The background color of a statement is proportional to the weight the model pays attention to it. %The box code is the source of the vulnerable statement.
%The red colored code in is the vulnerable statements.

\label{vul_example}
\end{figure}

\subsection{Why Does \tool Work?}
We identify %have identified 
the following advantages of \tool, which can explain its effectiveness in code vulnerability detection:

%\begin{itemize}
\textbf{(1) A simplified code structure graph.} {The proposed graph simplification methods reduce the node distance and code structure graph size, which can help \tool more effectively extract global information. As shown in Figure~\ref{distance}, compared with the original code structure graph, the average node distance and maximum node distance on three datasets drop by 41.65\% and 39.68\%, respectively. %As shown in Figure~\ref{cs_result}, the average node simplification rate and the average edge simplification rate on three datasets are as high as 41.64\% and 16.79\%, respectively. 
Figure~\ref{cs_result} also shows that the numbers of nodes and edges are reduced after simplification. 
}%The proposed graph simplification operations reduce the size of code structure graphs. 
%{\pan{As shown in Figure~\ref{cs_result}}
%As shown in Table~\ref{cs_result},         , compared with the original code structure graphs, the average edge compression ratio and the average node compression ratio on three datasets are as high as 16.79\% and 41.64\%, respectively.} \yun{[@yupan: to add.]}
     %of the simplified code structure graphs 
     %\hy{can use some data in Section 5 to support it} It makes it easier for GNNs to learn global information in code while preserving as many semantics as possible. 

\textbf{(2) The ability to handle graphs with multiple edge types.} We design the EA-GCN %edge-aware GCN 
module for heterogeneous multi-relational code graphs. It can produce the edge-enhanced node representation matrix, which incorporates
% contains 
the edge information in the simplified code structure graph. As shown in Table \ref{table_rq5}, the EA-GCN %edge-aware GCN  
module has significant advantages over all the other GNN models, with an average improvement of 2.39\% and 7.40\% in accuracy and F1 score, respectively.
     %On DELTA without Edge-Aware GCN module, the average loss of accuracy and F1 score on three datasets is 4.21\% and 6.92\% respectively, as  shown inTable \ref{table_rq5}. %\hy{can use some data in Section 5 to support it}

\textbf{(3) Better detection of code vulnerabilities by focusing on distant graph nodes.}
% Unlike traditional GNNs, \tool establishes node-to-node connections by capturing global information on the basis of capturing local information. Therefore, it is better able to identify graphs with a high number of nodes.
%2) \textbf{Effect of the number of graph nodes}
%GNNs-based methods are usually trained with \gsz{fewer}\hy{a few? a small number of?} %few
%layers \cite{zhu2021pre}, which \gsz{makes them}
Existing GNN-based methods often focus more on local information and ignore the global information in a graph. 
%We compare our proposed \tool with Devign on the Reveal dataset to further analyze the relationship between model performance and the number of graph nodes. 
As shown in Figure~\ref{discussion}, our \tool improves the accuracy in all intervals. In particular, when the number of nodes in the code structure graph is between (100, 150], \tool has a 25\% improvement compared with Devign. 
The results indicate that our method can better capture the global information in the code structure graph than previous methods.

To understand whether \tool
%Finally, to help understand whether the model 
pays attention to the vulnerable statements in the code, we illustrate the heatmap of attention for one example of CWE-77~\cite{CWE-77} in Figure~\ref{vul_example}. 
% displays a 
% heatmap of attention for a CWE-77~\cite{CWE-77} example, which % In the heatmap, %\pan{red-shaded statements are most contributing to the correct classification.}
Statements with higher attention weights are shaded in red.
Following Reveal~\cite{reveal}, we obtain the node importance by using an activation function. The activation values of each statement and its corresponding sub-AST nodes are summed as the statement's `attention' weight. Lines 8-9 are vulnerable statements and the heatmap shows that \tool focuses more on Line 8. %the vulnerability is lines 8 and 9. 
%\tool has the highest concern for line 8. 
Since the code in Lines 4-9 has strong semantic dependencies with Lines 8 and 9, these lines also receive relatively higher
% high 
attention, which
% . It 
enables \tool to make the accurate detection (\ie classifying the code as vulnerable).
%The result indicates that our method can not only pay more attention to the local information but also capture the global information in the code graph.  %means 
%that our method can captures the global information in the code graph while paying more attention to the local information (Section \ref{Kernel-scaled}).
%\end{itemize}







%\hy{explain why the proposed approach works. If possible, could give 1-2 cases as well. Could also move some descriptions in Section 5 here} 

%\subsection{Threats to Validity}
\subsection{Threats and Limitations}
%\hy{say some threats}
The first threat to validity is about the limited number of experimental datasets. {We evaluate \tool on three datasets: FFMPeg+Qemu, Reveal, and Fan \et. The main reason is that these three datasets are commonly used by previous related work \cite{devign, reveal,IVDETECT} on vulnerability detection.} %\hy{say these are commonly-used by related work, etc}
{Although these datasets cover many different types of open source projects, we will experiment with more datasets to further evaluate the effectiveness of \tool in our future work. }
%\pan{Although these datasets cover many different open-source projects and \tool performs well, future work can be extended to more other datsets to verify \tool.}
%The first threat to validity is about the bias in the numbers of different types of vulnerabilities. There is no specific vulnerability type in the training set and test set.
%\hy{not clear}% The number distribution information of different types \hy{not clear}of vulnerabilities is lacking in the training set and test set, 
%so the accuracy and F1 score can only reflect the overall performance of DELTA. %There may be few or no vulnerabilities of a certain type in the training set, which leads to poor performance of DELTA on this type of vulnerability. 
%Although our study is based on large numbers of datasets, future work can be extended to code with specific types of vulnerability.

The second threat to validity is that our proposed graph simplification is specific
% only applicable 
to C/C++ languages.  
%To alleviate the difficulty of GNN in capturing the global information of large graphs, we introduce two methods to reduce the complexity of the code structure graphs. Although experiments confirm the effectiveness of these two methods, there may be other graph simplification methods that can further condense the code structure graph. We will explore more graph simplification methods in our future work. 
We only conduct experiments on C/C++ datasets, and do not validate on datasets of other programming languages, such as Java and C\#. In the future, we will select datasets in more programming languages to verify our approach.


%\yun{[@xincheng: add threat]} 
%Finally, 
The third threat to validity is the implementation of baselines. Since Devign~\cite{devign} does not publish their implementation and hyper-parameters, we
reproduce the Devign based on the Reveal's~\cite{reveal} implementation.
%epository at $https://github.com/saikat107/Devign$. 
We try our best to tune its parameters as much as we can.
%We only experiment on C/C++ programs in three datasets, without differentiating between types of code vulnerabilities. 
%In the future, our approach can be easily extended to other programming languages.}
%The second threat to validity is about the simplified code structure graph. In graph condensing, we merge some nodes and simplify the parent-child edges. These operations change the original code structure graph and may affect the code representation learning of DELTA. Besides, the code structures extracted by Joern \cite{cpg} might not be reliable \cite{devign} and could influence the generated code structure graph. However, the accuracy and reliability is out of our study in this paper, and the effectiveness of Joern has been demonstrated in \cite{reveal}. 
%\hy{see if you have another threats to validity (replacing the second threat)}

%\hy{are experimental dataset and implementations  also a threat?}

==> sections/experimentalresult_old.tex <==
\subsection{RQ1. {Effectiveness of \tool}}
\input{tables/rq1.tex}
To answer the first question, we compare \tool{} with the six baseline methods with the four performance metrics (i.e., accuracy, precision, recall, and F1 score) on the three datasets. 
Table \ref{table_rq1} shows the results. 
The performance of \tool is shown in the bottom row. 
The best result for each performance metric is highlighted in bold. 
%We do not compare \tool with \ivd on Reveal and Fan \et. datasets, because \ivd sets the positive and negative samples in the training set to 1:1 and fails to converge on the unbalanced datasets of Reveal and Fan \et.



We observe that \tool outperforms all the baseline methods on the three datasets in terms of accuracy and F1 score. 
Specifically, \tool{} achieves 4.75\%, 6.86\%, and 9.24\% absolute improvement in F1 score over the best baseline method on the three datasets, respectively. 
The corresponding relative improvements are 7.63\%, 16.48\%, and 40.40\%. When considering all the four performance metrics regarding the three datasets (12 combination cases altogether), \tool{} has the best performance in 10 out of the 12 cases, and top-3 performance in 11 out of the 12 cases. 

% The performance of the baseline methods highly depends on the datasets and the metrics.
% For example, Reveal has the best baseline performance on the FFmpeg+Qemu dataset, but its performance on Fan \et. is relatively poor.

VulDeePecker, Russell \et., and SySeVR each have a metric value that beats \tool{}, but the superiority is on only one dataset, with poor performance on the remaining metrics.

% We also observe that \tool{}, together with other GNN-based methods, tend to have worse performance on the dataset of Fan \et. than on the other two datasets. This is because \jie{can we explain the reason? }
\wxc{Our results also show that the graph-based model methods mainly outperform existing work that uses token-based model methods. It is similar to the findings of many recent studies. This is because graph model-based approaches better capture structural information in the code (\eg, the data flow graph tracks the usage of variables.), which helps the model to improve the performance of code vulnerability detection.}

% \begin{tcolorbox}
% \textbf{Answer to RQ1:} \tool outperforms all the baseline methods in terms of accuracy and F1 score in software vulnerability detection. 
% In particular, \tool{} achieves 7.63\%, 16.48\%, and 40.40\% improvements in F1 score over the best baseline  method on the three datasets, respectively. 
% \end{tcolorbox}



\subsection{RQ2. Effectiveness of the Graph Simplification}
To answer the second research question, we first 
explore the contribution of the graph simplification to the performance of \tool{} and the effectiveness of different simplification methods. \pan{We also calculate the graph simplification rate (i.e., the ratio of reduced nodes and edges in code structure graphs) and the node distance (i.e., average node distance and maximum node distance) reduced by the two simplification methods. }
%then compare the simplified graphs and the original graphs to investigate the graph simplification rate (i.e., the ratio of reduced nodes and edges in code structure graphs).

\subsubsection{Impact on Model Performance}
\label{sec:graphsimplicationcontribution}

To evaluate the contribution of the graph simplification and the effectiveness of our proposed simplification methods, we perform an ablation study on three datasets. 
In particular, we compare the performance of four versions of \tool{}: without graph simplification (denoted as $Graph_{Original}$), with only \pan{TGS} %type-based graph simplification
(denoted as $Graph_{\namei}$), with only \pan{VGS} %variable-based graph simplification 
($Graph_{\nameii}$), and with both graph simplification methods ($Graph_{\final}$, the default \tool{}).

\input{tables/rq2.tex}

Table \ref{table_rq2} shows the \pan{ablation} results. The best result for each metric in the dataset is highlighted in bold. \pan{Compared with $Graph_{Original}$, $Graph_{\final}$ improves the accuracy by 6.58\%, 5.36\%, and 6.00\% on three datasets respectively, and improves the F1 by 12.56\%, 14.20\%, and 34.86\% respectively. Both $Graph_{\namei}$ and $Graph_{\nameii}$ outperform $Graph_{Original}$ in terms of accuracy and F1 on three datasets, which demonstrates our proposed graph simplification methods can facilitate the performance of \tool{}. In addition, $Graph_{\nameii}$ slightly outperforms $Graph_{\namei}$ since $Graph_{\nameii}$ improves the accuracy by 4.30\% and F1 by 2.92\% on average, while $Graph_{\namei}$ improves the accuracy by 3.40\% and F1 by 2.32\% on average. We suspect that
some variable nodes which gain more connected edges through VGS may play a key role in global representation learning.} %Compared with the model trained on the original code structure graphs (shown by the top row), the graph simplification (shown by the bottom row) improves the accuracy by 6.58\%, 5.36\%, and 6.00\% on three datasets respectively, and improves the F1 by 12.56\%, 14.20\%, and 34.86\% respectively. %In addition, $Graph_{\final}$ also increases F1 score by 12.56\%, 12.44\% and 21.92\%, respectively. %\pan{The results demonstrate that the graph simplification can facilitate the performance of \tool{}.} %The results demonstrate that the graph simplification plays an important role in the performance of \tool{}. % that our graph simplification module can reduce nodes while {preserving} semantic information, %maintaining % %as much semantic information as possible, % which helps subsequent DL modules to better understand the global information underlying the structure of the graph.% %can effectively reduce redundant nodes in the graph. %\pan{Table~\ref{table_rq2} also shows that each simplification method }               %Table~\ref{table_rq2} also shows that although the combination of the two simplification strategies yields the best performance, each single simplification strategy is helpful to improve model performance.         %$Graph_{\namei}$ and $Graph_{\nameii}$ yield an average improvement of 3.40\% and 4.30\% regrading F1 respectively, and 2.32\% and 2.92\% in accuracy. %Thus, $Graph_{\nameii}$ slightly outperforms $Graph_{\namei}$ in accuracy and F1 score.  %We suspect that this is because \nameii              %\jie{following explanation is unclear to me}              %reduces the nodes while preserving the structure of AST. Using both methods simultaneously %rather than one               %can relieve noisy nodes to a greater extent. Therefore, the experiment results are also better. The results demonstrate that extracting features of our simplified code structure graph %with larger information density %is significantly more effective for detecting vulnerabilities. %\subsection{RQ3. What is the impact of the individual modules of \tool?}
\subsubsection{Graph Simplification Rate}
\label{sec:simplicationrate}
\jie{Jie will revise this part afterwards}
We also investigate how many nodes and edges can our graph simplification module reduces for the code structure graphs.
Figure~\ref{cs_result} shows the box-whisker plot of node simplification rate (i.e., the ratio of reduced nodes) and edge simplification rate (i.e., the ratio of reduced edges) on each dataset. \wxc{The average simplification rate is the average of the simplification rates for each graph.}
%\jie{following sentence unclear to me}The average simplification ratio is obtained by calculating the average of the simplification ratios of each graph. 

\begin{figure}[t]
   
	\centering

	\includegraphics[width=0.5\textwidth]{figures/rq2_rate_cropped.pdf}
	\caption{Edge simplification ratio and node simplification ratio on three datasets. \final represents the final simplified code structure graph after type-based graph simplification and variable-based graph simplification.}
    \label{cs_result}
\end{figure}


From the figure we can find that the average node/edge simplification ratio of type-based graph simplification is higher than that of variable-based graph simplification, which indicates that there are more redundant nodes in the AST than the nodes of the same variable. {Specifically, the average node simplification and edge simplification ratio of the final simplified code structure graph on the three datasets is 41.64\% and 16.79\%, respectively. } 

%In addition, we can also find that the ratio of simplified nodes is higher than that of edges. Before simplification, a node connects to 1.62 edges on average while after simplification the average edges for a node is 2.21.

%This results indicate that the information in simplified code structure graph is more dense.

\begin{figure}
    \centering
    \subfloat[Average node distance]{
    \begin{minipage}[t]{0.46\linewidth}
    \centering
    \includegraphics[width=1.0\textwidth]{figures/compressionresult_cropped.pdf}

    %\caption{fig2}
    \label{Avg}
    \end{minipage}%
    }
    \hspace{1mm}
    \vspace{-1mm}
    \subfloat[Maximum node distance]{
    \begin{minipage}[t]{0.46\linewidth}
    \centering
    \includegraphics[width=1.025\textwidth]{figures/compressionresult_cropped (1).pdf}
    %\caption{fig2}
    
    \label{Max}
    \end{minipage}
    }
\centering
\caption{Average node distance and maximum node distance on the test set of FFmpeg+Qumu, Reveal and Fan \et. %CSG, TGS, VGS and SCSG represent the original code structure graph, code strucutre graph with TGS, code structure graph with VGS and code structure graph with both simplification methods respectively. 
The y-axis represents the node distance which is measured by the length of the shortest path between two nodes.
}
\end{figure}



%\jie{please add comparison analysis cross different datasets}

%\jie{please give examples of extreme cases such as those that got significantly simplified and those that cannot be simplified.}
%压缩情况

% \begin{tcolorbox}
% \textbf{Answer to RQ2:} TBD 
% \end{tcolorbox}


\subsection{\wxc{RQ3. Effectiveness of Enhanced Graph Representation Learning}
}

To answer the third research question. In this section, we explore the impact of the enhanced graph representation learning in \tool. As mentioned in Section~\ref{sec:framework}, \tool consists of the edge-aware graph convolutional network module (EA-GCN) and the \ksr(\ksrab).

\subsubsection{Edge-aware Graph Convolutional Network Module}
To explore the contribution of the edge-aware graph convolutional network module, we create a variant that does not contain edge-aware graph convolutional network module, which directly feed the simplified code structure graph into \ksrab module. The rest of the settings for this variant are consistent with \tool.

As shown in Table \ref{table_rq3}, we can observe that the edge-aware graph convolutional network module significantly improves the performance of code vulnerability detection. For the F1 score, it achieves a performance improvement over the variant on all datasets, e.g., 4.46\% in FFMPeg+Qemu, 30.08\% in Reveal, and 48.66\% in Fan \et., repectively. Although the variant in the Devign dataset improves the recall by 0.64\%, it also sacrifice the precision of 7.83\%, 
which shows that the edge-aware graph convolutional network module focus more on the different relations in graph structure. As a result, the edge-aware graph convolutional network module can improve the performance of vulnerability detection.
\input{tables/rq3.tex}

To further explore the effectiveness of the edge-aware graph convolutional network module, we replace the module with other existing GNN models, including GCN \cite{kipf2016gcn}, GGNN \cite{Method3}, R-GCN \cite{Method5} and compare them with %the performance 
of \tool. As shown in Table \ref{table_rq5}, the edge-aware graph convolutional network module obtains significant improvements on all databases. In particular, compared to the other best performing GNN methods, the F1 score metric improved by 6.78\%, 15.48\% and 39.12\% on the three datasets, respectively. The edge-aware graph convolutional network is modified from R-GCN and uses a multi-head attention to weight the importance representation of different relationships. It can effectively enhance the distinction between different edge types in simplified code structure graph and greatly improve the performance.
\input{tables/rq5.tex}

%We argue that the edge-aware graph convolutional network module not only embeds the node information of its neighbors into each vertex through neighbor aggregation but also focuses more on the different types of edge information in the graph structure so that the vertices have richer information about the CPG. As a result, the edge-aware graph convolutional network module can be used for higher performance in code vulnerability detection tasks. \wxc{To be modified}

\subsubsection{Kernel-scaled Representation Module}\label{kscr}

To understand how the \ksr works, we also deploy a variant of \tool without this module. 

The variant directly employs a classifier to replace the \ksr to classify the edge-enhanced node feature matrix.
Table \ref{table_rq3} also shows the performance of the above setup on the three datasets. On all three datasets, better performance is obtained with the addition of the \ksr. Specifically, the F1 score is 13.13\%, 57.53\%, and 27.93\% of \tool higher than that of the variant on FFMPeg+Qemu, Reveal, and Fan \et. datasets. Meanwhile, \tool increases the accuracy by 11.22\%, 17.15\%, and 4.69\% compared with the variant on the three datasets, respectively. These results demonstrate that our \ksrab module brings a significant performance improvement.

% \begin{tcolorbox}
% \textbf{Answer to RQ3:} The performance of vulnerability detection can be effectively contributed by using enhanced graph representation learning. It can build the relations between distant graph nodes and capture global information.
% \end{tcolorbox}

\subsection{\wxc{Influences of Hyperparameter Tuning}}

\begin{figure}[t]
	\centering

	\includegraphics[width=0.3\textwidth]{figures/conv_cropped.pdf}
	\caption{Impact of
% 	the large and small 
	kernel sizes on the performance of \tool. \pan{The x-axis and y-axis indicate the small kernel size and large kernel size respectively.} %The x-axis indicates the size of the small kernel, and the y-axis indicates the size of the large kernel. 
	The darker the color, the better the performance.}
	\label{fi_conv}

\end{figure}

%\subsubsection{The Size of Convolutional Kernel}
%In addition to the two modules mentioned above, we also explore the impact of the sizes of two branch convolution's kernels on the performance.
\wxc{To answer the fourth research question, we explore the impact of different hyperparameter tuning, including the sizes of two branch convolution kernel, the layer number of the e-aware graph convolutional
network module and the head number of the attention.}

\subsubsection{\wxc{Sizes of Two Branch Convolution Kernel}}
%In Figure~\ref{fi_conv}, the x-axis represents the size of the small convolution kernel, while the y-axis represents the size of the large convolution kernel, and the magnitude of the value indicates the corresponding F1 score size. for a small convolutional kernel size of 3 and a large convolutional kernel of 11.
\wxc{Figure~\ref{fi_conv} shows that \tool achieves the highest F1 score for a small convolutional kernel of 3 and a large kernel of 11}. When both large and small convolution kernels use the same kernel size, relatively low F1 scores are achieved. The results indicate that using one type of convolutional kernel does not capture the global and local information well. We argue that in the two branch convolution, the large kernel branch is more inclined to capture global information, while the small kernel convolution is more focused on the extraction of local information. Besides, due to the limited number of nodes in the simplified code structure graph, the size of the large kernel branch cannot be increased infinitely and the F1 score starts to decrease at kernel size = 13.
In short, the model benefits from a larger kernel size and meanwhile retains the capability of capturing local information in the graph structure from a small kernel size. It captures the relations between distant graph nodes, which is beneficial for learning the global information of graphs.

\subsubsection{\wxc{Layers of Edge-aware GCN's}}

We also conduct a study of the impact of other hyperparameters on \tool. We also use Devign's dataset as an example, Table\ref{hyper} shows the results of the \wxc{edge-aware graph convolutional layers}. For other datasets, \tool exhibits similar trends.  In particular, using a 2-layer e-aware graph convolutional network module obtains the accuracy of 62.16\% and F1 of 66.94\%. As the number of layers continues to increase, GNNs experience over-smoothing~\cite{bottleneck}. This makes the model lose the information about the neighborhood, leading to the degradation of performance.

\subsubsection{\wxc{Heads of attention}} Besides, using more heads instead of a single head brings a noticeable improvement in accuracy. It shows that understanding different edge information and diverse structural information in the code structure graph from multiple aspects helps improve model's performance. However, employing more than 10 heads does not further improve accuracy.

% \begin{tcolorbox}
% \textbf{Answer to RQ4:} We conduct a study of the impacts of hyper-parameters on \tool.
% \end{tcolorbox}


%The results show that the prediction performance for the code vulnerability task is improved by using both the beater and small convolution to some extent, taking into account the extraction of both global and local information.
\input{tables/hyper.tex}

%\subsection{RQ4. How does Edge-aware Graph Convolutional Network module compare to other existing GNN models in code vulnerability detection?}
%\subsection{RQ4. Is the proposed Edge-aware Graph Convolutional Network module effective?}

% {To explore the effectiveness of the Edge-aware Graph Convolutional Network module proposed in this paper, we replace the module with an existing GNN model (including GCN \cite{kipf2016gcn}, GGNN \cite{Method3}, R-GCN \cite{Method5}) and compare the resulting performance of \tool. As shown in Table \ref{table_rq5}, edge-aware Graph Convolutional Network module obtains a significant improvement on all databases. In particular, the F1-score metric improved by 4.25\%, 5.75\% and 5.95\% on the three databases respectively.  Edge-aware Graph Convolutional Network is modified from R-GCN and uses a multi-head attention to weight the importance representation of different relationships among code nodes. It can effectively enhance the distinction between different edge types in simplified code structure graph and greatly improve the performance.}

% \subsection{RQ4. How do different training data splitting ratio affect \tool’s performance?}

% In the real world, it is a common phenomenon that there are more non-fragile code examples in the dataset than fragile examples. This can lead to training models in datasets with this tendency to be easily biased, overly favoring the category with more examples. For example, we find that IVDETECT performs poorly for code vulnerability detection in the Reveal dataset (9.17\% share of vulnerability classification) and the Fan et al. dataset (5.88\% share of vulnerability classification). Therefore, IVDETECT uses a new data partitioning approach, which first uses the true ratio between vulnerable and non-vulnerable samples in the original dataset divided into 8:1:1. For training, only the same number of non-vulnerable and vulnerable samples are used to obtain balanced training data. For validation and test data, the true ratio from the original dataset is used. In this RQ, we evaluate our method in this same way. It is worth mentioning that the validation and test data in this type of division are kept consistent with the experimental ones in RQ1.

% Table \ref{table_rq4} shows the metrics at the above mentioned division ratios. We observe that \tool exhibits better performance in all cases, regardless of the division. Compared to the previous state-of-the-art work, the model brings 6.04\%, 5.45\% and 1.5\% improvement in F1-score, respectively. There are similarly notable improvements in Accuracy and Precision, with an average improvement of 9.17\% and 4.35\%. However, our method does not perform well on Recall, and is in the middle of the pack on both Reveal and Fan. We believe that, compared to the true proportional division, even if a more balanced training data is obtained in the training leads to not overly favoring one class in the process of recognition. However, the missing data still contains some useful information. As a result, the model will not be able to extract more useful information and will instead learn some of the redundant information. The results show that after using balanced data partitioning, the performance for code vulnerability detection is in a degraded situation for all cases except IVDETECT on FFmpeg+Qemu database.


%\pan{\tool achieves an average F1 score improvement of 13.82\% on the three datasets compared to all baseline methods.[xx]}
%\tool achieves an average F1 score improvement of 15.03\% on FFMPeg+Qemu compared to all baseline methods.
% The relative average gain of F1 score is 4.75\%, 6.11\% and 6.16\%, compared with the previous best performing approach Reveal on the %FFmpeg+Qemu, Reveal and Fan et al. 
% three datasets, respectively. 
% Specifically, compared with the previous state-of-the-art baseline Reveal, \tool outperforms it by 4.75\%, 6.11\%,  and 6.16\% with respect to the F1 score on three datasets, respectively.
% {In addition, \tool improves the \wxc{Reveal} by 1.09\%, 2.65\% and 0.04\% in terms of accuracy on the three datasets.}

%In addition, the accuracy of \tool is increased  by 1.09\% (compared with Reveal), 2.65\% (compared with Devign) and 0.04\% (compared with Devign) on the three datasets. 
% Note that %our approach is not compared with
% {we do not compare \tool with} IVDETECT on Reveal and Fan et al. datasets, %for this class division. 
% {because IVDETECT sets the positive and negative samples in the training set to 1:1 and }
% %\wxc{Because IVDETECT uses a balanced training set division, where the  ratio of positive to negative samples in the training data is 1:1, which } 
% fails to converge %under popular data division 
% on the unbalanced datasets of Reveal and Fan et al. 
% To conclude, \tool outperforms the previous state-of-the-art vulnerability detection methods on all datasets




% evaluate %illustrate 
% the effectiveness of our graph simplification module in simplifying code structure graph from two aspects, including simplification rate and its impact on the model performance.}
% We illustrate the advantages of our proposed Graph Simplification module from two aspects: simplification rate and performance.

% \begin{figure}[t]
% 	\centering
	
%     \includegraphics[width=0.52\textwidth]{figures/conv2_new_cropped.pdf}
%     \vspace{-4px}
% 	%\includegraphics[width=11cm]
% 	\caption{The Effective Receptive Field (ERF) Visualisation of (a) small convolutional kernel and  (b) large convolutional kernel. More widely distributed dark area indicates a larger ERF. It can be found that larger convolution kernels are easily and efficiently obtained with larger ERFs.}%\hy{this part could be omitted if space is a concern}}
% 	\label{fi_conv1}

% \end{figure}

%generates a larger effective receptive field (ERF) than traditional small-kernel convolution.
% defined as a measure of the region~\cite{erf} of interest of the features of a given convolution in the input space. the larger the ERF, the larger the range of information that can be understood by the convolution.

% In addition to evaluating the effectiveness of the module, we also explore the effect of the large kernel. We visualize convolution's effective receptive field (ERF), which is related to the ability of features to capture information. A larger ERF value means that the model can better capture global information and the connections between different nodes in the graph.
% Figure~\ref{fi_conv1} (a) and (b)represent the ERF of the small convolutional kernel and large convolutional kernel, respectively. We can observe that the small kernel has only the least perceptual field and is not sensitive to context information.
% In contrast, the effective field of perception increases obviously with a large kernel, demonstrating that the model can better capture the contextual structural information.
% Compared with other baselines approaches, the kernel-scaled code representation module can have a larger ERF than others, which makes the model to better capture the global information.


%Our proposed kernel-scaled code representation module has a larger ERF than the (a) network structure containing only small convolutions. It means that our module extract more global information in graph. 

% of the context. 
% We also analyze the ERF with multi-layer convolutional kernels, as shown in Figure~\ref{fi_conv1} (c). 
% But as shown in Section 5.3.3, even though it has a larger ERF, the model may learn some redundant information in global information, which leads to degradation in classification performance. 

%Compared with other approaches, the kernel-scaled code representation module can have a larger ERF than others, which makes the model more sensitive to global information. 
%In summary, \tool is able to better capture global information, which is helpful for improving the performance of vulnerability detection.


%Compared with other GNN approaches, the kernel-scaled code representation module can have a larger ERF than others, which makes the model more sensitive to global information. Therefore, KCR can better handle the connections between different code nodes and thus

% Meanwhile, the Kernel-Scaled code representation module uses shortcuts to benefit from a larger perceptual field while ensuring that the ability to capture local information in the graph structure is not lost. }
%We suggest that the module uses large convolution to expand the perceptual field and learn more global information from the graph data. The module uses both reparameterisation and shortcuts to benefit from a larger perceptual field while ensuring that the ability to capture local information in the graph structure is not lost.  \wxc{To be modified}

==> sections/graphcompress_last.tex <==
%\usepackage{xr}
%\externaldocument{experimentalresult}
%\yun{to add}
\subsection{Graph simplification module} \label{GraphSimplification}

%In this section, we introduce two methods of code graph simplification, which can help reduce the redundant information in CPG and debase the complexity of graphs. 
%{In this section, we describe the details of the graph simplification module, which can be divided into two parts:}

%\wxc{The detailed process is shown in Algorithm \ref{algorithm1}, which successively simplified the extracted code structure graph with \csi and \csii.}
% Our experiment performances show that these two simplification methods are effective, and the detailed overall simplification degree on each dataset is shown in Fig.\ref{cs_result}

%\hy{why after compression, you can still detect vulnerabilities?}

\begin{figure}[t]
\centering
\includegraphics[width=0.40\textwidth]{figures/TGS_cropped.pdf}
% \vspace{-2ex}
\caption{An example illustrating \namei (Type-based Graph Simplification). %The first line of text in each graph node represents the code value, and the second line of text represents the type. 
{The text in each node represents the node value and the text under the node represents the node type. }Some nodes and edges are omitted {for facilitating illustration}. The node with red dashed border in the top original code strucutre graph is merged with its parent node, producing a TGS-based simplified graph.}%\hy{can remove the three ''down arrows'' in the bottom of the two figures? rather confusing}}
\label{cs_1}
\end{figure}


%Following the previous work \cite{devign, reveal}, we produce a code property graph by extracting the structures of AST, CFG and DFG via Joern \cite{cpg}. Next, we connect all of the leaf nodes of AST to reflect the source code sequence. We adopt this approach and add the NCS (Natural Code Sequence) edge to the code graph. 

\pan{To reduce the distances between nodes in the code structure graph, we propose graph simplification module that contains two methods: type-based graph simplification and variable-based graph simplification. These two methods shrink the sizes of code graph structures according to the node type attribute and node variables respectively. In the following, we introduce the  type-based graph simplification , variable-based graph simplification, and a detailed algorithm about graph simplification module.}
%The graph simplification module is proposed to shrink the size of code structure graphs while preserving the code semantic information. 
%It can be divided into two parts:
%The two simplification methods are: 
%\textit{\textbf{T}ype-based \textbf{G}raph \textbf{S}implification} and \textit{\textbf{V}ariable-based \textbf{G}raph \textbf{S}implification}. 

% and names this type of edge $NCS$ (Natural Code Sequence). To reserve the programming logic reflected by the source code sequence, we also add NCS.} 

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=8.0cm]{figures/source_Code.png}
%\vspace{-2ex}
%\caption{Code Example with Buffer Overflow}
%\label{source_code}
%\end{figure}

%\begin{figure*}[h]
%	\centering
%	\includegraphics[width=18cm]{../figures/ori_graph.png}
%	\caption{Overview of the whole CPG.}
%	\label{CPG}
%\end{figure*}
\subsubsection{Type-based Graph Simplification}
 \namei is a method for merging adjacent nodes of specific node types. %\namei determines whether a node can be condensed according to its type information.
 \pan{According to the parsing principles of Joern~\cite{}, we randomly select 50 code structure graphs from the three datasets and manually summarize the attributes of the nodes that can be merged. }
 %\pan{which is based on the hypothesis: the node which value is repetitive with the value of its parent node and which type is included into the type of its parent node can be merged to the parent node, since it does not add additional value information to the code structure graph. }
 %After examining numerous\jie{vague: how many graphs have you examined?} code structure graphs generated by Joern, we notice that merging some\jie{vague: which nodes?} adjacent nodes would not cause the loss of {too much} node value information\jie{vague: how did you measure information loss? How much loss will be caused?} in AST. %\hy{what do PType and CType mean? what are they for? need explanations}
 For example, for the code shown in Figure~\ref{cs_1}, we merge the node with red dashed border to its parent node for two reasons: (1) The type of the parent node (in the red box) is ``\textit{IdentifierDeclStatement}'' indicating variable declaration, while the type ``\textit{Identifierdecl}'' of its child node is a structural refinement of ``\textit{IdentifierDeclStatement}''.  (2) Although the child node ``\textit{* first = malloc(10)}'' does not contain the variable type ``char'' in its code value, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type. Therefore, the basic {syntactic structure information can be preserved after} deleting this child node and connecting the grandchild nodes to the parent node.

{We use \textit{(PType, CType)} to indicate the types of adjacent nodes that can be merged, 
 %the types of such node pairs, 
 where \textit{PType} and \textit{CType} denote the type of the parent node and child node, respectively}. %The first three authors spent two weeks summarizing (PType, CType) from a large number of code structure graphs, including real-world functions in the dataset and synthesized functions of various basic syntax in C/C++.\hy{not necessary}} 
 Table \ref{type} shows the identified $(PType, CType)$ pairs\jie{this is important: please explain how you identified the pairs in the table, details needed}. 
 For the cases 1-5, \namei %needs to 
checks whether the types of two adjacent nodes match the (PType, CType).
For the cases 6-8, there are two conditions to be satisfied: (1) the parent node type conforms to PType, and (2) the code values of the parent node and the child node are equal. {In case 6, the ``Argument'' type represents the parameters of function call statements, which child node type further describes the specific type of the parameter and can be of various types (\eg array, constant) and usually has the same value with the parent node.}
%When traversing the graph, 
During graph traversal, when each time encountering a pair of adjacent nodes $(u,v)$ conforming to the condition of $(PType, CType)$, the following operations are performed:  deleting $v$ and the edges connected with $v$, adding a new edge $(u, r)$ with the same type as $(v, r)$ where $r$ $\in$ neighbor($v$) and $r$ $\neq$ $u$. If the types of $(v, r)$ also match $(PType, CType)$, we also delete $r$ and the edges connected to $r$, and connect the neighbor nodes of $r$ to $u$. {In this way, for each pair of adjacent nodes matching $(PType, CType)$, the type of the child node is a refinement of the parent node type, and the value of the child node is part of the parent node value. The merging operation will not lose too much node value information and can reduce the depth of AST hierarchy.}
%\hy{can briefly explain why they can be merged. (and why the 6 rules are identified)}

% {For the example in Figure~\ref{cs_1}, we merge the node with red dashed border to its parent node for two reasons: (1) The type of the parent node (in the red box) is ``\textit{IdentifierDeclStatement}'' indicating variable declaration, while the type ``\textit{Identifierdecl}'' of its child node is a structural refinement of ``\textit{IdentifierDeclStatement}''.  (2) Although the child node ``\textit{* first = malloc(10)}'' does not contain the variable type ``char'' in its code value, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type. }
% %The type of node in the red box is ``\textit{IdentifierDeclStatement}'' indicating a sentence of variable declaration, while the type of its child node is ``\textit{Identifierdecl}'', which is a structural refinement of ``\textit{IdentifierDeclStatement}''
% %Compared with the parent node, the child node ``\textit{* first = malloc(10)}'' does not contain the variabTGSle type ``char'' in its code value. However, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type
% Therefore, the basic {syntactic structure information can be preserved after}
% % can keep unchanged when
% deleting this child node and connecting the grandchild nodes to the parent node.
% % deleting this child node and connecting the grandchild nodes to the parent node can maintain the basic syntactic structure. 


\begin{figure}[t]
\centering

\includegraphics[width=0.5\textwidth]{figures/VGS_cropped.pdf}
% \vspace{-4ex}
\caption{An example illustrating \nameii (Variable-based Graph Simplification). The node with red dashed border in the top original code structure graph is merged to the  previous node ``str'', producing a VGS-based simplified code structure graph, as shown in the bottom graph.}%The dotted line with red cross shows the situation of repeatedly considering `str` node when constructing NCS edge, which results in a directed cycle.
\label{cs_2}
\end{figure}

\subsubsection{Variable-based Graph Simplification}
{\nameii is a method for merging nodes by the node value. The same variable in a function often appears many times, resulting in repeated appearance in the code structure graph. }
%After \csi, there %is a 
%{still exits a} problem that the same variable often appears repeatedly in a function, which leads to {node} duplication %of nodes 
%in the graph. 
%Thus, we condense the graph according to the {code value} of the node. 
In this work, we propose \nameii to remove the duplicate variable nodes in a code structure graph and only keep the nodes that first appear in the function\jie{need more explanation on why this does not affect code semantics}. {\nameii only applies to the leaf nodes of AST and does not change the edge numbers, therefore it preserves the structure of AST as much as possible. }% \nameii ensures that each variable will appear only once in the code graph.
% \pan{After \csi, we condense the graph according to the value attribute of the node.}
%\wxc{After the process of \csi, we condese the value attributed of node.} 
% The same variable often appears repeatedly in a function, resulting in duplicate nodes in the code graph. \nameii is to remove the duplicate variable nodes in a code graph and only keep the ones that first appear in the function. This method ensures that each variable will appear only once in the code graph.
%\wxc{The variable can be captured via the merged repeated nodes and the structural information is retained via the parent-child edges. And the more complex edge representation after the change is focused on the edge-aware graph convolutional network module.}
%\hy{does this kind of  compression affect vulnerability detection?}

%Fig.\ref{cs_2} is the part of code graph after  \namei.
Figure~\ref{cs_2} presents an example of %the process of 
\nameii. %on the graph.
In the statement ``\textit{scanf(''\%s'',str);}'', the variable ``\textit{str}'' has appeared in the AST expansion of the ``\textit{char str[15]; }'' node. So we merge the ``\textit{str}'' node of ``\textit{scanf(''\%s'',str);}'' into that of ``\textit{char str[15]; }''. %It is worth noting that \nameii only applies to the leaf nodes of AST. For instance,  $(...,v_i,...,v_k,v_j,v_t,...)$ is the original AST leaf nodes sequence, where $v_i$ and $v_j$ represent the same variable. After \nameii merging $v_j$ to $v_i$, the sequence becomes $(...,v_i,...,v_k,v_t,...)$. %, {Thus} the NCS edge path is constructed as: $(... \to v_i \to ... \to v_k \to v_t \to ...)$.
%The NCS edges are: $(... \to v_i \to ... \to v_k \to v_t \to ...)$. 


%There are two ways to construct NCS edges after variable merging. The first is to connect leaf nodes in the original order.% This connection will lead to the directed cycle. 
%The first is to repeatedly connect $v_i$ when constructing NCS edges. Directed cycles will appear in the NCS edges obtained in this way: $(v_i \to ... \to v_k \to v_i \to v_t \to ...)$, as shown by the dashed line with red cross in Fig.\ref{cs_2}.
%Another way is to delete the repeated leaf nodes from the original order. 
%Another way is not to repeatedly connect nodes $v_i$: $(v_i \to ... \to v_k \to v_t \to ...)$. 
%In order to reduce the complexity of the graph, we use the second method.

\subsubsection{The Algorithm {of} Graph Simplification}
\jie{In Section III.B, we need to first introduce the overall algorithm, then introduce the details for the two parts of simplification.}
The detailed process is shown in Algorithm \ref{algorithm1}, which simplifies the extracted code structure graph with type-based graph simplification and variable-based graph simplification. The algorithm takes the node set $V$ and edge set $E$ of the function extracted by Joern as the input, and outputs the simplified code structure graph. The algorithm initializes an empty set $SCSG$ to store the edges of the simplified code structure graph at the beginning (Line 1). It first searches all AST edges: takes each statement node in $V$ as the root to obtain a subtree through traversing $E$, and add it to $ast\_edges$ (Lines 2-8). The next loop performs type-based graph simplification (Lines 9-11). The algorithm carries out breadth-first traversal on each subtree in $ast\_edges$, and each time the types of two adjacent nodes conforms to Table \ref{type}, the child nodes are merged into the parent nodes. The algorithm obtains leaf nodes in $ast\_edges$ and searches the same variable groups according to code value (Lines 12-13). The next loop is about variable-based graph simplification (Lines 14-21). The main operation is to merge the leaf nodes in each subtree into the first nodes of the same variable groups where the leaf nodes are located. Finally, the algorithm adds AST, NSC, CFG and DFG edges to $SCSG$ and outputs $SCSG$ (Lines 22-26).
%\hy{describe a bit about the algorithm. Like lines xx-yy do this, yy-zz to that}

% \begin{algorithm}[ht] 
% \caption{Algorithm for the graph simplification module} 
% \label{GraphCompress} 
% \begin{algorithmic}[1]
% \REQUIRE ~~\\ %算法的输入参数：Input
% V: node set of the function; \\
% E: edge set of the function;
% \ENSURE ~~\\ %算法的输出：Output
% \textit{SCSG}: the final graph after simplification;%, a list with triple elements:[s,e,t], s and t are edge vertices, e is the edge type.
% \STATE $\textit{SCSG}\gets\varnothing$ %\quad $\backslash$$\backslash$ for storing the final code graph after \namei and \nameii;
% \STATE $\textit{ast\_edges} \gets \varnothing$ %\quad$\backslash$$\backslash$ for storing all the original AST edges;
% % \Comment{This is a comment}
% \FOR{each $v \in V$}
% \IF{v represents a statement node }
% \STATE $T_v \gets $ \ generate an abstract syntax tree with v as the root node.\\ \STATE $\textit{ast\_edges} \gets \textit{ast\_edges} \bigcup T_v$
% \ENDIF
% \ENDFOR
% %\STATE $\backslash$$\backslash$\namei
% %\STATE $\textit{ast\_edges\_1}\gets\varnothing$ \quad $\backslash$$\backslash$ for storing all the AST edges after \namei;
% \FOR{each $T \in \textit{ast\_edges}$} 
% \STATE Perform breadth first traversal of T. Each time the types of a pair of adjacent nodes conform to Table \ref{type}, merge the child node into the parent node;
% \ENDFOR
% \STATE $\textit{leaf\_nodes} \gets $\ get all the  leaf nodes involved in \textit{ast\_edges}
% \STATE $\textit{same\_variable} \gets$\ get all the node groups with the same code value in \textit{leaf\_nodes}
% %\STATE $\backslash$$\backslash$\nameii
% \FOR{each $T \in \textit{ast\_edges}$}
% \STATE $\textit{leaves} \gets$ \ get all the leaf nodes in T
% \FOR{each $v \in \textit{leaves}$}
% \IF{$v \in \textit{same\_variable}$}
% \STATE Merge v to the first node in the node group where v is located;
% \ENDIF
% \ENDFOR
% \ENDFOR
% \STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup \textit{ast\_edges}$
% \STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup NCS$\ edges
% \STATE $\textit{other\_edges} \gets $\ traverse E to obtain edges of CFG type and DFG type;
% \STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup \textit{other\_edges}$ 
% \STATE Return \textit SCSG;
% \end{algorithmic} 
% \label{algorithm1}
% \end{algorithm}

% \begin{algorithm}[!tpb]
%     \SetAlgoLined
%     \footnotesize
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \SetKwFunction{Simplification}{Simplification}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Input{Code Structure Graph -- \textit{CSG}}
%     \Output{Simplified Code Structure Graph -- \textit{SCSG} }
%     \Fn{}{\For{each AST \textbf{T} in  \textit{CSG}}
%     {\For{each pair of adjacent nodes (u,v) \in \textbf{T}}{
%     \If{u.Type \&\& v.Type conform to (PType, CType)}{Merging v to u;}}}
    
    
%     }
%       $leaf\_nodes$ \leftarrow $\varnothing$ \\
%       \For{each AST \textbf{T} in \textit{CSG}}{}
    
% \end{algorithm}

\begin{algorithm}[!tpb]
    \SetAlgoLined
    \footnotesize
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}
    \SetKwFunction{Simplification}{Simplification}
    \SetKwProg{Fn}{Function}{:}{}
    \Input{Original Code Structure Graph -- ${Graph_{original}}$}
    \Output{Simplified Code Structure Graph -- ${Graph_{SCSG}}$ }
    \Fn{}{
    \tcp{The procedure of type-based graph simplification.} \tcp{$Graph_{TGS}$ denotes the graph after type-based graph simplification. }
    \For{each AST \textbf{T} in  \textit{CSG}}{
    \If{u.Type \&\& v.Type conform to (PType, CType)}{
    Merging node v to node u;
    }
    }
    \tcp{The procedure about variable-based graph simplification.}
    $leaf\_nodes \leftarrow$ get all the leaf nodes of AST in  $Graph_{TGS}$\\
    $same_{variable} \leftarrow$ get all the node groups with the same code value in $leaf\_nodes$ \\
    \For{each AST \textbf{T} in $Graph_{TGS}$}{
    $leaves \leftarrow$ get all the leaf nodes in \textbf{T} \\
    \For{each $v \bigcup leaves$ }{
    \If{$v \bigcup same_{variable}$}{
    Merging $v$ to the first node in the node group where $v$ is located.
    }
    }
    
    }
    return $Graph_{SCSG}$

    }
    \caption{\textbf{\small Algorithm for the graph simplification module.}}
    \label{algo}
\end{algorithm}


% \begin{algorithm}[!tpb]
%     \SetAlgoLined
%     \footnotesize
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \SetKwFunction{SMOTE}{SMOTE}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Input{Training Dataset -- $\mathbb{D}_\text{train}$\\
%           Number of Nearest Neighbors -- $k$, \\
%           Expected Number of samples per class -- $m$
%          }
%     \Output{Sampled Dataset -- $\mathbb{D}_\text{sampled}$.}
%     % \Fn{\Fframework{$\mathbb{D}_\text{train}, \alpha, \beta, \gamma, lr$}}{
%     \Fn{\SMOTE{$\mathbb{D}_\text{train}$, $k$, $m$}}{
%         $\mathbb{D}_\text{sampled} \leftarrow \mathbb{D}_\text{train}$\\
%         \While{\# of Majority examples $> m$}{
%             $x \leftarrow $ random majority class example from $\mathbb{D}_\text{sampled}$\\
%             Remove $x$ from $\mathbb{D}_\text{sampled}$\\
%         }
%         \While{\# of Minority examples $< m$}{
%             $x \leftarrow $ random minority class example from $\mathbb{D}_\text{sampled}$\\
%             $neighbors \leftarrow k$ nearest minority neighbors of $x$\\
%             \For{$n \in neighbors$}{
%                 $x_s \leftarrow interpolate(x, n)$\\
%                 Add $x_s$ to $\mathbb{D}_\text{sampled}$\\
%             }
%         }
%         \Return  a %$\mathbb{D}_\text{sampled}$\\
%     }
%     \caption{\textbf{\small Algprithm for SMOTE.}\hy{is it standard SMOTE? if so can omit the algorithm} \pan{}}
%     \label{alg:smote}
% \end{algorithm}






==> sections/graphcompress_old.tex <==
%\usepackage{xr}
%\externaldocument{experimentalresult}
%\yun{to add}
\subsection{Graph simplification module} \label{GraphSimplification}
%In this section, we introduce two methods of code graph simplification, which can help reduce the redundant information in CPG and debase the complexity of graphs. 
%{In this section, we describe the details of the graph simplification module, which can be divided into two parts:}

%\wxc{The detailed process is shown in Algorithm \ref{algorithm1}, which successively simplified the extracted code structure graph with \csi and \csii.}
% Our experiment performances show that these two simplification methods are effective, and the detailed overall simplification degree on each dataset is shown in Fig.\ref{cs_result}

%\hy{why after compression, you can still detect vulnerabilities?}

\begin{figure}[t]
\centering
\includegraphics[width=0.40\textwidth]{figures/TGS_cropped.pdf}
% \vspace{-2ex}
\caption{An example illustrating \namei (Type-based Graph Simplification). %The first line of text in each graph node represents the code value, and the second line of text represents the type. 
{The text in each node represents the node value and the text under the node represents the node type. }Some nodes and edges are omitted {for facilitating illustration}. The node with red dashed border in the top original code strucutre graph is merged with its parent node, producing a TGS-based simplified graph.}%\hy{can remove the three ''down arrows'' in the bottom of the two figures? rather confusing}}
\label{cs_1}
\end{figure}


%Following the previous work \cite{devign, reveal}, we produce a code property graph by extracting the structures of AST, CFG and DFG via Joern \cite{cpg}. Next, we connect all of the leaf nodes of AST to reflect the source code sequence. We adopt this approach and add the NCS (Natural Code Sequence) edge to the code graph. 


The graph simplification module is proposed to shrink the size of code structure graphs while preserving the code semantic information. It can be divided into two parts:
%The two simplification methods are: 
\namei (\textit{\textbf{T}ype-based \textbf{G}raph \textbf{S}implification}) and \nameii (\textit{\textbf{V}ariable-based \textbf{G}raph \textbf{S}implification}). 

% and names this type of edge $NCS$ (Natural Code Sequence). To reserve the programming logic reflected by the source code sequence, we also add NCS.} 

%\begin{figure}[htbp]
%\centering
%\includegraphics[width=8.0cm]{figures/source_Code.png}
%\vspace{-2ex}
%\caption{Code Example with Buffer Overflow}
%\label{source_code}
%\end{figure}

%\begin{figure*}[h]
%	\centering
%	\includegraphics[width=18cm]{../figures/ori_graph.png}
%	\caption{Overview of the whole CPG.}
%	\label{CPG}
%\end{figure*}
\subsubsection{\csi}
 \namei is a method for merging adjacent nodes of specific node types. %\namei determines whether a node can be condensed according to its type information.  
 After examining numerous\jie{vague: how many graphs have you examined?} code structure graphs generated by Joern, we notice that merging some\jie{vague: which nodes?} adjacent nodes would not cause the loss of {too much} node value information\jie{vague: how did you measure information loss? How much loss will be caused?} in AST. %\hy{what do PType and CType mean? what are they for? need explanations}
 For example, for the code shown in Figure~\ref{cs_1}, we can merge the node with red dashed border to its parent node for two reasons: (1) The type of the parent node (in the red box) is ``\textit{IdentifierDeclStatement}'' indicating variable declaration, while the type ``\textit{Identifierdecl}'' of its child node is a structural refinement of ``\textit{IdentifierDeclStatement}''.  (2) Although the child node ``\textit{* first = malloc(10)}'' does not contain the variable type ``char'' in its code value, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type. Therefore, the basic {syntactic structure information can be preserved after} deleting this child node and connecting the grandchild nodes to the parent node.

{We use \textit{(PType, CType)} to indicate the types of adjacent nodes that can be merged, 
 %the types of such node pairs, 
 where \textit{PType} and \textit{CType} denote the type of the parent node and child node, respectively}. %The first three authors spent two weeks summarizing (PType, CType) from a large number of code structure graphs, including real-world functions in the dataset and synthesized functions of various basic syntax in C/C++.\hy{not necessary}} 
 Table \ref{type} shows the identified $(PType, CType)$ pairs\jie{this is important: please explain how you identified the pairs in the table, details needed}. 
 For the cases 1-5, \namei %needs to 
checks whether the types of two adjacent nodes match the (PType, CType).
For the cases 5-7, there are two conditions to be satisfied: (1) the parent node type conforms to PType, and (2) the code values of the parent node and the child node are equal. {In case 6, the ``Argument'' type represents the parameters of function call statements, which child node type further describes the specific type of the parameter and can be of various types (\eg array, constant) and usually has the same value with the parent node.}
%When traversing the graph, 
During graph traversal, when each time encountering a pair of adjacent nodes $(u,v)$ conforming to the condition of $(PType, CType)$, the following operations are performed:  deleting $v$ and the edges connected with $v$, adding a new edge $(u, r)$ with the same type as $(v, r)$ where $r$ $\in$ neighbor($v$) and $r$ $\neq$ $u$. If the types of $(v, r)$ also match $(PType, CType)$, we also delete $r$ and the edges connected to $r$, and connect the neighbor nodes of $r$ to $u$. {In this way, for each pair of adjacent nodes matching $(PType, CType)$, the type of the child node is a refinement of the parent node type, and the value of the child node is part of the parent node value. The merging operation will not lose too much node value information and can reduce the depth of AST hierarchy.}
%\hy{can briefly explain why they can be merged. (and why the 6 rules are identified)}

% {For the example in Figure~\ref{cs_1}, we merge the node with red dashed border to its parent node for two reasons: (1) The type of the parent node (in the red box) is ``\textit{IdentifierDeclStatement}'' indicating variable declaration, while the type ``\textit{Identifierdecl}'' of its child node is a structural refinement of ``\textit{IdentifierDeclStatement}''.  (2) Although the child node ``\textit{* first = malloc(10)}'' does not contain the variable type ``char'' in its code value, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type. }
% %The type of node in the red box is ``\textit{IdentifierDeclStatement}'' indicating a sentence of variable declaration, while the type of its child node is ``\textit{Identifierdecl}'', which is a structural refinement of ``\textit{IdentifierDeclStatement}''
% %Compared with the parent node, the child node ``\textit{* first = malloc(10)}'' does not contain the variabTGSle type ``char'' in its code value. However, the leftmost grandchild node ``\textit{char *; IdentifierType}'' of the parent node reflects the variable type
% Therefore, the basic {syntactic structure information can be preserved after}
% % can keep unchanged when
% deleting this child node and connecting the grandchild nodes to the parent node.
% % deleting this child node and connecting the grandchild nodes to the parent node can maintain the basic syntactic structure. 


\begin{figure}[t]
\centering

\includegraphics[width=0.5\textwidth]{figures/VGS_cropped.pdf}
% \vspace{-4ex}
\caption{An example illustrating \nameii (Variable-based Graph Simplification). The node with red dashed border in the top original code structure graph is merged to the  previous node ``str'', producing a VGS-based simplified code structure graph, as shown in the bottom graph.}%The dotted line with red cross shows the situation of repeatedly considering `str` node when constructing NCS edge, which results in a directed cycle.
\label{cs_2}
\end{figure}

\subsubsection{\csii}
{\nameii is a method for merging nodes by the node value. The same variable in a function often appears many times, resulting in repeated appearance in the code structure graph. }
%After \csi, there %is a 
%{still exits a} problem that the same variable often appears repeatedly in a function, which leads to {node} duplication %of nodes 
%in the graph. 
%Thus, we condense the graph according to the {code value} of the node. 
In this work, we propose \nameii to remove the duplicate variable nodes in a code structure graph and only keep the nodes that first appear in the function\jie{need more explanation on why this does not affect code semantics}. {\nameii only applies to the leaf nodes of AST and does not change the edge numbers, therefore it preserves the structure of AST as much as possible. }% \nameii ensures that each variable will appear only once in the code graph.
% \pan{After \csi, we condense the graph according to the value attribute of the node.}
%\wxc{After the process of \csi, we condese the value attributed of node.} 
% The same variable often appears repeatedly in a function, resulting in duplicate nodes in the code graph. \nameii is to remove the duplicate variable nodes in a code graph and only keep the ones that first appear in the function. This method ensures that each variable will appear only once in the code graph.
%\wxc{The variable can be captured via the merged repeated nodes and the structural information is retained via the parent-child edges. And the more complex edge representation after the change is focused on the edge-aware graph convolutional network module.}
%\hy{does this kind of  compression affect vulnerability detection?}

%Fig.\ref{cs_2} is the part of code graph after  \namei.
Figure~\ref{cs_2} presents an example of %the process of 
\nameii. %on the graph.
In the statement ``\textit{scanf(''\%s'',str);}'', the variable ``\textit{str}'' has appeared in the AST expansion of the ``\textit{char str[15]; }'' node. So we merge the ``\textit{str}'' node of ``\textit{scanf(''\%s'',str);}'' into that of ``\textit{char str[15]; }''. %It is worth noting that \nameii only applies to the leaf nodes of AST. For instance,  $(...,v_i,...,v_k,v_j,v_t,...)$ is the original AST leaf nodes sequence, where $v_i$ and $v_j$ represent the same variable. After \nameii merging $v_j$ to $v_i$, the sequence becomes $(...,v_i,...,v_k,v_t,...)$. %, {Thus} the NCS edge path is constructed as: $(... \to v_i \to ... \to v_k \to v_t \to ...)$.
%The NCS edges are: $(... \to v_i \to ... \to v_k \to v_t \to ...)$. 


%There are two ways to construct NCS edges after variable merging. The first is to connect leaf nodes in the original order.% This connection will lead to the directed cycle. 
%The first is to repeatedly connect $v_i$ when constructing NCS edges. Directed cycles will appear in the NCS edges obtained in this way: $(v_i \to ... \to v_k \to v_i \to v_t \to ...)$, as shown by the dashed line with red cross in Fig.\ref{cs_2}.
%Another way is to delete the repeated leaf nodes from the original order. 
%Another way is not to repeatedly connect nodes $v_i$: $(v_i \to ... \to v_k \to v_t \to ...)$. 
%In order to reduce the complexity of the graph, we use the second method.

\subsubsection{The Algorithm {of} Graph Simplification}
\jie{In Section III.B, we need to first introduce the overall algorithm, then introduce the details for the two parts of simplification.}
The detailed process is shown in Algorithm \ref{algorithm1}, which simplifies the extracted code structure graph with type-based graph simplification and variable-based graph simplification. The algorithm takes the node set $V$ and edge set $E$ of the function extracted by Joern as the input, and outputs the simplified code structure graph. The algorithm initializes an empty set $SCSG$ to store the edges of the simplified code structure graph at the beginning (Line 1). It first searches all AST edges: takes each statement node in $V$ as the root to obtain a subtree through traversing $E$, and add it to $ast\_edges$ (Lines 2-8). The next loop performs type-based graph simplification (Lines 9-11). The algorithm carries out breadth-first traversal on each subtree in $ast\_edges$, and each time the types of two adjacent nodes conforms to Table \ref{type}, the child nodes are merged into the parent nodes. The algorithm obtains leaf nodes in $ast\_edges$ and searches the same variable groups according to code value (Lines 12-13). The next loop is about variable-based graph simplification (Lines 14-21). The main operation is to merge the leaf nodes in each subtree into the first nodes of the same variable groups where the leaf nodes are located. Finally, the algorithm adds AST, NSC, CFG and DFG edges to $SCSG$ and outputs $SCSG$ (Lines 22-26).
%\hy{describe a bit about the algorithm. Like lines xx-yy do this, yy-zz to that}

\begin{algorithm}[ht] 
\caption{Algorithm for the graph simplification module} 
\label{GraphCompress} 
\begin{algorithmic}[1]
\REQUIRE ~~\\ %算法的输入参数：Input
V: node set of the function; \\
E: edge set of the function;
\ENSURE ~~\\ %算法的输出：Output
\textit{SCSG}: the final graph after simplification;%, a list with triple elements:[s,e,t], s and t are edge vertices, e is the edge type.
\STATE $\textit{SCSG}\gets\varnothing$ %\quad $\backslash$$\backslash$ for storing the final code graph after \namei and \nameii;
\STATE $\textit{ast\_edges} \gets \varnothing$ %\quad$\backslash$$\backslash$ for storing all the original AST edges;
\FOR{each $v \in V$}
\IF{v represents a statement node }
\STATE $T_v \gets $ \ generate an abstract syntax tree with v as the root node.\\ \STATE $\textit{ast\_edges} \gets \textit{ast\_edges} \bigcup T_v$
\ENDIF
\ENDFOR
%\STATE $\backslash$$\backslash$\namei
%\STATE $\textit{ast\_edges\_1}\gets\varnothing$ \quad $\backslash$$\backslash$ for storing all the AST edges after \namei;
\FOR{each $T \in \textit{ast\_edges}$} 
\STATE Perform breadth first traversal of T. Each time the types of a pair of adjacent nodes conform to Table \ref{type}, merge the child node into the parent node;
\ENDFOR
\STATE $\textit{leaf\_nodes} \gets $\ get all the  leaf nodes involved in \textit{ast\_edges}
\STATE $\textit{same\_variable} \gets$\ get all the node groups with the same code value in \textit{leaf\_nodes}
%\STATE $\backslash$$\backslash$\nameii
\FOR{each $T \in \textit{ast\_edges}$}
\STATE $\textit{leaves} \gets$ \ get all the leaf nodes in T
\FOR{each $v \in \textit{leaves}$}
\IF{$v \in \textit{same\_variable}$}
\STATE Merge v to the first node in the node group where v is located;
\ENDIF
\ENDFOR
\ENDFOR
\STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup \textit{ast\_edges}$
\STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup NCS$\ edges
\STATE $\textit{other\_edges} \gets $\ traverse E to obtain edges of CFG type and DFG type;
\STATE $\textit{SCSG} \gets \textit{SCSG} \bigcup \textit{other\_edges}$ 
\STATE Return \textit SCSG;
\end{algorithmic} 
\label{algorithm1}
\end{algorithm}






==> sections/relatedwork.tex <==


% Deep-learning based vulnerability detection aims to automatically accumulate the experience of identifying vulnerabilities from a large number of datasets. It can not only mitigate the labor burden of auditors, but also help discover new vulnerabilities, which can be served as an auxiliary of traditional program analysis methods. The goal of vulnerability detection using deep learning is to learn a mapping function: $f:x \to y$, $x$ is a code element and $y$ is the corresponding label, 0 means non-vulnerable and 1 means vulnerable. Supposing that there are n functions in the training set, f can be obtained by minimizing the loss function: $\sum_{i=1}^{n}\Gamma(f(x_i),y_i)$, $\Gamma$ can be the cross entropy loss function.

% Two key points for the task of DL-based vulnerability detection are the choice of neural network and how to represent the code into an input suitable for the model. 2.1 and 2.2 respectively introduce the solutions of existing code vulnerability detection work in code representation learning and graph neural network models.
%\hy{maybe can combine Related Work here...}

% \pan{There have been a wide array of vulnerability detection research on source code which can be divided into two categories: similarity-based and pattern-based. }

% \pan{\subsection{Similarity-Based Vulnerability Detection}}


% \pan{}

% \pan{\subsection{Pattern-Based Vulnerability Detection}}

%In this section, we introduce the related work about code representation and deep learning in vulnerability detection.

\subsection{Code Representation in Vulnerability Detection}

In recent years, many {code representation learning-based} vulnerability detection methods~\cite{vuldeepecker,devign,duan2019vulsniper,220} have been proposed.
%based on the neural representation of source code.
These research works %in representation learning of source code 
can be divided into two categories: sequence-based approaches and structure-based approaches. {Several early works \cite{vuldeepecker,russell, dam2017automatic} regard the source code as flat sequences and adopt natural language processing techniques to segment the code snippets and initialize the token vectors with Word2Vec \cite{wv}.} This processing method has no requirements for code integrity and syntax correctness. But due to the neglect of the inherent structural regularity,
%\hy{structural regularity?}. % and inner logicality, 
it could obtain shallow %and superficial 
code semantics, thereby leading to {poor} %sub-optimal 
detection performance. {To leverage tree structures of AST,} Lin et al. \cite{lin2018cross} and POSTER \cite{lin2017poster} serialize AST into sequences through depth-first traversal to add syntactic knowledge to code representation. 
Allamanis et al. \cite{allamanis2017learning} combine AST and DFG to represent programs. They argue that explicitly exposing code structural semantics to the model helps improve data quality. SySeVR \cite{sysevr} and IVDETECT \cite{IVDETECT} utilize PDG structure in the graphs. 
Devign \cite{devign}, ReVeal \cite{reveal} and VulSniper \cite{duan2019vulsniper} leverage code structure graph, a comprehensive graph composed of AST, CFG, and DFG, to capture code semantic information from multiple aspects. The studies show that graph structure, especially joint graph structure, can promote code representation learning.
% We detail the GNN-based vulnerability detection literature in Section~\ref{subsec:gnn}.
% \gsz{We will introduce the details of graph neural networks-based vulnerability detection methods in the next section.}%\wcz{However, the complexity of the graph leads to low space efficiency and increases the time consumption, which is unacceptable to apply in large-scale software.}


\subsection{Deep Learning in Vulnerability Detection}\label{subsec:gnn}
% Graph Neural Networks
%\hy{maybe Graph Neural Networks in Vulnerability Detection}
%The neural networks used in the existing literature mainly include:CNN(Convolutional Neural Network), RNN(Recurrent neural Network) and GNN(Graph Neural Network). Russell\cite{russell} input the lexical code representation into CNN. Vuldeepecker\cite{vuldeepecker} employed BLSTM to handle code gadget, a fine-grained code slice. Xi Gong et al \cite{gong2019joint}, SySeVR\cite{sysevr} also selected LSTM.  RNNs are suitable for processing serialized information, while most of those who learn code representations from code graphs choose GNN. IVDetect\cite{IVDETECT} explored vulnerability explainability based on GCN(Graph Convolutional Network). They constructed the PDG but did not use edge type information. Devign\cite{devign}, Reveal\cite{reveal} and FUNDED\cite{9293321} used GGNN\cite{Method3} to model multiple code relationships from source code. GGNN regards the relationship graph as multiple directed graphs, which can capture more complex edge relationships in different nodes. %However, it shares the same parameters in each iteration and fails to perform hierarchical feature extraction.

%For function-level vulnerability detection task, incorporating both structure features and contextual information in code representation will further facilitate the model performance. For contextual information, although CNN can project words contained in the context window to local contextual features, it cannot learn the structure information. 
%Although CNN can capture contextual information by controlling context windows, it cannot learn the structure information. 
%However, when considering graph structure, GGNN can not take into account the context information, since in each iteration, the current node focuses on the local structure, generally one-hop neighbor nodes. 
%And when GGNN updates the node feature, the current node focuses on the local structure, generally one-hop neighbor nodes. 
%We hope to increase convolution to capture local information and global information concurrently and make them interact when passing message. 
%We hope to capture deeper global and local information in high-level features by enlarging the form of effective receptive field in convolution. Through the interaction between global and local information, the impact of this information on the results is captured

The neural networks used in the existing works mainly include CNN (Convolutional Neural Network) \cite{russell}, RNN (Recurrent Neural Network) \cite{gong2019joint,sysevr}, and GNN (Graph Neural Network) \cite{devign, reveal}.
%\gsz{Recently, GNN-based methods have gained substantial attention and achieved state-of-the-art performance on vulnerability detection.[Is this claim strict?]}
Russell et al.\cite{russell} input the lexical code representation into CNN. Vuldeepecker \cite{vuldeepecker} employs BiLSTM to handle the code gadgets, a fine-grained code slice. Some work \cite{gong2019joint,sysevr} also selects LSTM as code encoders. 
{ While RNNs are suitable for processing sequence data, there are a series of studies learning code representations from code graphs via GNN.}
Devign \cite{devign}, Reveal \cite{reveal} and FUNDED \cite{9293321} 
{leverage} GGNN \cite{Method3} to model multiple code relationships from source code. GGNN regards the relationship graph as multiple directed graphs, which can capture more complex edge relationships in different nodes. However, as GGNN shares the same parameters in each iteration, it fails to perform hierarchical feature extraction. Meanwhile, for function-level vulnerability detection task, GGNN tends to obtain graph representation vectors on top of node vectors. We argue that extracting high-level features from the CPG with both graph structure and node feature information can better facilitate code vulnerability detection.

Li et al. \cite{IVDETECT} explore vulnerability explainability based on GCN (Graph Convolutional Network). Their proposed IVDETECT considers the contextual information between neighboring nodes by adding a neighboring statement vector. {However, it} is still not effective to understand the contextual information of the overall graph structure.
{In %our 
{this} work, we aim to capture deeper global and local information in high-level features by enlarging the form of the effective receptive field (ERF)~\cite{erf} in convolution. An ERF is a region containing nodes with a non-negligible impact on the target node. The number of nodes that the network focuses on depends on the size of the ERF.} %\hy{cite, also can explain what it is} 
Through the interaction between global and local information, the performance of vulnerability detection can be significantly improved. 

%Meanwhile, GGNN tends to obtain the graph representation based on the node vectors

==> sections/relatedwork_old.tex <==



%To recap the state-of-the-art of software vulnerability detection researches, we introduce the related work from……

There have been significant vulnerability detection researches based on DL. Russell. et al \cite{russell} explored both CNNs and RNNs for feature extraction directly from source code. VulDeePecker \cite{vuldeepecker} and SySeVR \cite{sysevr} constructed slices containing multiple lines of code that were semantically related to each other and utilized LSTM to learn representations. These above works regarded the source code as flat sequences and adopted the technology similar to natural language processing to segment the code and initialized the token vectors with Word2Vec \cite{wv}. And due to the neglect of the inherent structure and inner logicality, they can only obtain shallow and superficial code semantics, thereby leading to less than ideal detection performance. 

To fully utilize the code structure information, many works \cite{devign, reveal, IVDETECT, 9293321} considered the code structure, such as Abstract Syntax Tree, Control Flow graph, Data Flow graph, Program Dependency graph and so on to promote the code representaion learning. And these works generally selected Graph Neural Network because of its advantages in capturing graph structures. Devign \cite{devign} augmented a new type of Natural Code Sequence (NCS) on CPG proposed by Yamaguchi et al. \cite{cpg} and used GGNN model with Gated Graph Recurrent Layers for graph classification. Reveal \cite{reveal} also utilized GGNN with Triplet Loss to learn graph representations from source code. Li et al. \cite{IVDETECT} learned representations for each of the five different types of code graphs and classified the program dependence graph (PDG) by FA-GCN \cite{Method4}. The dominant position of GNNs in code vulnerability detection has been proved. However, they are sensitive to local information and lack the ability to capture global information. Our proposed model can effectively fuse the global information and local information. %While capturing global information through deepening network is expensive in time and hardware, our proposed model can effectively capture global information at low cost.

%With the rapid development of deep learning in recent years, more and more researchers are applying dl-based methods to source code vulnerability detection. Most researchers first used source code as a natural language sequence. Natural language sequences had strong temporal and contextual characteristics, and architectures such as RNN and LSTM are most broadly applied. For example, in 2018, Russel et al.\cite{russell} treated source code as a token sequence and automatically used RNNs to extract source code features for vulnerability detection. However, such methods only learned the source code semantically and sequentially, mainly ignoring the code's expression logic and structural information. Therefore, Zhou et al.\cite{devign} used graph neural networks to solve this task to exploit better different types of graph properties in the source code, which vastly improved the performance of code vulnerability detection. Later, Chakraborty et al.\cite{reveal} proposed to use of gated graph neural networks to learn graph properties from source code. Li et al.\cite{IVDETECT} learned representations for each of the five different types of code graphs and classified the program dependence graph (PDG) by FA-GCN. Although these studies have shown good performance on function-level vulnerability detection tasks, some problems still exist. On the one hand, the code graph structure contains a lot of partially redundant information, resulting in low performance in vulnerability prediction. On the other hand, most of the work focuses too much on graph properties and ignores the contextual information in the code, so there is still much room for improvement in the function-level vulnerability detection task.

==> tables/rq4.tex <==
% \begin{table*}[]
% \centering

% \setlength{\tabcolsep}{1.2mm}
% \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{c|cccc|cccc|cccc}
% \toprule
% \diagbox{Baseline}{Dataset} & \multicolumn{4}{c|}{FFmpeg+Qemu}        & \multicolumn{4}{c|}{Reveal}             & \multicolumn{4}{c}{Fan et al.}                \\
% \midrule
% Metrics(\%)                         & Accuracy & Precision & Recall & F1     & Accuracy & Precision & Recall & F1     & Accuracy & Precision & Recall & F1     \\

% \midrule
% Devign                          & 54.42   & 49.87    & 65.41 & 56.59 & 73.19   & 17.17    & 51.28 & 25.72 & 78.38   & 11.32    & 41.41 & 17.17 \\

% Reveal                          & 54.96   & 55.05    & 60.20 & 57.51 & 72.53   & 18.45    & \textbf{57.55} & 27.94 & 68.84   & 10.40    & 58.17 & 17.64 \\

% IVDETECT                        & 56.21   & 51.70    & 66.13 & 58.03 & 80.80   & 27.57    & 55.62 & 36.86 & 68.45   & 11.87    & \textbf{59.87} & 19.82 \\
% \midrule
% Our proposed                    & \textbf{61.55}   & \textbf{55.50}    & \textbf{75.77} & \textbf{64.07} & \textbf{89.20}   & \textbf{35.26}    & 52.88 & \textbf{42.31} & \textbf{82.15}   & \textbf{13.42}    & 51.74 & \textbf{21.32}\\
% \bottomrule
% \end{tabular}
% \caption{The performance comparisons on the FFmpeg+Qemu, Reveal, and Fan et al. datasets in Li's\cite{IVDETECT} division method}
% \label{table_rq4}
% \end{table*}

==> tables/type_new.tex <==
\newcommand{\tabincell}[3]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\begin{table}[]
\centering

\begin{tabular}{|c|c|c|}
\hline
case 	& parent	 & child    \\
\hline
\multirow{4}{*}{1} & \multirow{4}{*}{ExpressionStatement} & AssignmentExpression          \\
                   &                                      & UnaryExpression               \\
                   &                                      & CallExpression                \\
                   &                                      & PostIncDecOperationExpression \\
\\
\hline
2		 &IdentifierDeclStatement & IdentifierDecl \\
\hline
3        &ForInit   & AssignmentExpression \\
\hline
4        & CallExpression      &ArgumentList  \\
\hline
5        &Callee    &Identifier \\
\hline
6        & Argument  &  *   \\
\hline
7        &Condition    &     *      \\
\hline
8        & ForInit   &     *      \\
\hline

\end{tabular}
\caption{(PType, CType) pairs. {*} represents any type.}
\label{type}
\end{table}


